Branch-Avoiding Graph Algorithms

This paper quantifies the impact of branches and branch mispredictions on the single-core performance for two classes of graph problems. Specifically, we consider classical algorithms for computing connected components and breadth-first search (BFS). We show that branch mispredictions are costly and can reduce performance by as much as 30%-50%. This insight suggests that one should seek graph algorithms and implementations that avoid branches. As a proof-of-concept, we devise such implementations for both the classic top-down algorithm for BFS and the Shiloach-Vishkin algorithm for connected components. We evaluate these implementations on current x86 and ARM-based processors to show the efficacy of the approach. Our results suggest how both compiler writers and architects might exploit this insight to improve graph processing systems more broadly and create better systems for such problems.

==> branchPred.tex <==
% New algorithm2e keywords
\SetKw{KwGoto}{goto}

% States of the Markov chain for a 2-bit branch predictor
\newcommand{\SNT}{\ensuremath{\xoverline{S}}\xspace}
\newcommand{\WNT}{\ensuremath{\xoverline{W}}\xspace}
\newcommand{\WT}{\ensuremath{W}\xspace}
\newcommand{\ST}{\ensuremath{S}\xspace}

% Probability notation
\newcommand{\Prob}[1]{\ensuremath{\mathrm{Pr}[#1]}\xspace}
\newcommand{\ProbText}[1]{\Prob{\mbox{\small #1}}}
\newcommand{\Expect}[1]{\ensuremath{E[#1]}\xspace}

% Probabilities of being in a given predictor state
\newcommand{\PrSNT}{\ensuremath{\xoverline{s}}\xspace}
\newcommand{\PrWNT}{\ensuremath{\xoverline{w}}\xspace}
\newcommand{\PrWT}{\ensuremath{w}\xspace}
\newcommand{\PrST}{\ensuremath{s}\xspace}
\newcommand{\PrStateVec}[1]{\ensuremath{\mathrm{\mathbf{#1}}^T}\xspace}
\newcommand{\PrStateVeci}[2]{\ensuremath{\mathrm{\mathbf{#1}}^T_{#2}}\xspace}
\newcommand{\PrVecP}{\PrStateVec{p}}
\newcommand{\PrVecQ}{\PrStateVec{q}}
\newcommand{\PrVecPfirst}{\PrStateVeci{p}{0}}
\newcommand{\PrVecPsecond}{\PrStateVeci{p}{1}}
\newcommand{\PrVecPthird}{\PrStateVeci{p}{2}}
\newcommand{\PrVecPfourth}{\PrStateVeci{p}{3}}
\newcommand{\PrVecPim}{\PrStateVeci{p}{i-1}}
\newcommand{\PrVecPi}{\PrStateVeci{p}{i}}
\newcommand{\PrVecPip}{\PrStateVeci{p}{i+1}}
\newcommand{\PrVecPlastTaken}{\PrStateVeci{p}{n-1}}
\newcommand{\PrVecPlast}{\PrStateVeci{p}{n}}

% Branch probabilities
\newcommand{\PrTaken}{\ensuremath{b}\xspace}
\newcommand{\PrTransMat}{\ensuremath{G_{\PrTaken}}\xspace}
\newcommand{\PrTransMatNT}{\ensuremath{G_{0}}\xspace}
\newcommand{\PrTransMatT}{\ensuremath{G_{1}}\xspace}

% Correct prediction events and probabilities
\newcommand{\CORR}{\ensuremath{C}\xspace} % Event ``correct prediction''
\newcommand{\INCORR}{\ensuremath{\neg C}\xspace} % Event ``incorrect prediction''
\newcommand{\CorrValue}[2]{\ensuremath{c_{#1}(#2)}\xspace}
\newcommand{\ExINCORR}{\ensuremath{E[\INCORR]}\xspace} % Expected value of an incorrect prediction

% Mispredictions symbol
\newcommand{\SingleBranchMispred}[1]{\ensuremath{\xoverline{M}(#1)}\xspace}
\newcommand{\SimpleLoopMispred}[2]{\ensuremath{\xoverline{M}_{#1}({#2})}\xspace}

Given a particular (static) conditional branch in a program, our analysis goal is to estimate how many times the predictor will mispredict it.
To do so, we model the predictor's behavior mathematically using a Markov chain.
This choice derives from the fact that most branch predictors use the history of a given conditional branch to predict what the next occurrence of the branch will do.
For instance, a simple \emph{1-bit} predictor predicts that if the last occurrence of a given branch was taken, then so will the next one.
This dependence on a finite-number of previous states suggests Markov chains are a suitable analysis tool.

Although we do not know exactly what type of branch predictor a vendor implements, our analysis assumes a \emph{2-bit branch predictor}~\cite{} (see \refsec{sec:2-bit}).
We then setup a Markov chain analysis of the 2-bit predictor and analyze the possible behaviors of different kinds of conditional branches (\refsec{sec:2-bit:model}).

\begin{figure}
  \includegraphics[width=\columnwidth,clip=true,trim=.5in 0in .5in 0in]{figs/branch-pred-fsa.pdf}
  \caption{
    A 2-bit branch predictor behaves as shown in this finite-state automaton.
    Each node is a state representing the next prediction, e.g., the strongly and weakly taken states predict ``taken,'' the others, ``not taken.''
    Each edge shows how the state changes once the actual branch condition is resolved.
  }
  \label{fig:branch-pred-fsa}
\end{figure}

\subsection{2-bit predictors}
\label{sec:2-bit}
For each (static) conditional branch in the program, a 2-bit predictor maintains a 2-bit state value, which encodes four possible states.
Each state value is a prediction for the next occurrence of this branch;
once the true branch condition is known, this state is updated.
The precise states and transitions appear in the finite-state automaton (FSA) of \reffig{fig:branch-pred-fsa}.
In particular, there are four possible states, named ``strongly taken,'' ``weakly taken,'' ``weakly not taken,'' and ``strongly not taken.''
The ``strong'' states reflect that the last few branches were all the same, i.e., all ``taken'' or all ``not taken,'' and so it is likely the next branch will be the same.
The weak states allow for the predictor's bias to change if a new pattern emerges.

\subsection{Model for a single branch}
\label{sec:2-bit:model}
Consider the conditional branch of \refalg{alg:1-branch}.
We wish to model the number of times that the branch predictor mispredicts it.
To do so, we interpret the 2-bit predictor's FSA (\reffig{fig:branch-pred-fsa}) as a Markov chain.

%------------------------------------------------------------
\begin{algorithm}[t]
\Indp
  \tcp*[h]{Predictor's initial state: \PrVecP} \;
  \lIf{(\textit{condition})}{\KwGoto{taken}}
    \Indp
    \BlankLine
    \tcp*[h]{\ldots~NOT TAKEN path~\ldots} \;
    \BlankLine
    \Indm
\Indm\Indm
\emph{taken}:\ \ \;
\Indp\Indp
  \tcp*[h]{Predictor's final state: \PrVecQ} \;
  \caption{Single conditional branch}
  \label{alg:1-branch}
\end{algorithm}
%------------------------------------------------------------

The nodes of \reffig{fig:branch-pred-fsa} becomes the state probabilities of the Markov chain.
Let $\PrVecP \equiv [\PrSNT, \PrWNT, \PrWT, \PrST]$ be a row-vector that represents the initial probabilities of being in one of the four possible prediction states just before we encounter the branch.
The values \PrSNT, \PrWNT, \PrWT, and \PrST are the probabilities of being in the strongly not taken, weakly not taken, weakly taken, and strongly taken states, respectively, and they must sum to 1.
When the processor encounters the conditional branch, we may assert that the predictor will, for instance, predict ``taken'' with probability $\PrWT + \PrST$, and ``not taken'' with probability $\PrSNT+\PrWNT=1-(\PrWT+\PrST)$.

Each edge $(u, v)$ in \reffig{fig:branch-pred-fsa} becomes a transition probability of changing to the destination state, $v$, from the source state $u$.
For instance, suppose we know the probability that the branch is taken, independent of the FSA's state, is \PrTaken.
Then, if $(u, v)$ is a ``taken'' edge, then $\ProbText{v|u}=\PrTaken$.
These edge probabilities define a probability transition matrix, \PrTransMat, such that the state of the predictor after the branch is resolved is $\PrVecQ=\PrVecP\PrTransMat$, where
\begin{eqnarray}
  \PrTransMat
    & = & \left(\begin{array}{cccc}
            1-\PrTaken &  \PrTaken  &     0      &     0      \\
            1-\PrTaken &      0     &  \PrTaken  &     0      \\
                0      & 1-\PrTaken &     0      &  \PrTaken  \\
                0      &      0     & 1-\PrTaken &  \PrTaken
          \end{array}\right).
\end{eqnarray}
%
This model immediately implies a useful fact.

\begin{lemma}
  Consider the single conditional branch of \refalg{alg:1-branch}.
  If a 2-bit conditional branch predictor begins in a state $\PrVecP = [\PrSNT, \PrWNT, \PrWT, \PrST]$ and the probability of taking the branch is \PrTaken, then the expected number of mispredictions, \SingleBranchMispred{\PrVecP}, is
%
  \begin{eqnarray*}
      \SingleBranchMispred{\PrVecP}
        & = & 1 - \CorrValue{\PrTaken}{\PrVecP} = \CorrValue{1 - \PrTaken}{\PrVecP} \\
    \mbox{where\ }
      \CorrValue{\PrTaken}{\PrVecP}
        & = & (\PrWT + \PrST)\PrTaken + \left[1 - (\PrWT + \PrST)\right](1 - \PrTaken).
  \end{eqnarray*}
%
\end{lemma}

\newcommand{\PREDT}{\ensuremath{K}\xspace}
\newcommand{\PREDNT}{\ensuremath{\neg K}\xspace}
\newcommand{\TAKEN}{\ensuremath{B}\xspace}
\newcommand{\NOTTAKEN}{\ensuremath{\neg B}\xspace}

\begin{proof}
To see this fact, begin by letting \PREDT be the Boolean random variable for the event, ``predicts taken,'' and let \TAKEN be the Boolean event, ``branch is taken,'' once the condition is resolved.
The prediction is \emph{correct} if it matches the branch, that is, the event $\CORR \equiv (\PREDT \wedge \TAKEN) \vee (\PREDNT \wedge \NOTTAKEN)$.
Thus,
%
\begin{eqnarray}
  \Prob{\CORR}
    & \equiv & \Prob{(\PREDT \wedge \TAKEN) \vee (\PREDNT \wedge \NOTTAKEN)} \nonumber \\
    & \equiv & \Prob{\PREDT \wedge \TAKEN} + \Prob{\PREDNT \wedge \NOTTAKEN} \nonumber \\
    & = & \Prob{\PREDT|\TAKEN}\Prob{\TAKEN} + \Prob{\PREDNT|\NOTTAKEN}\Prob{\NOTTAKEN} \\
    & = & (\PrWT + \PrST)\PrTaken + (\PrSNT + \PrWNT)(1 - \PrTaken) \\
    & = & (\PrWT + \PrST)\PrTaken + \left[1 - (\PrWT + \PrST)\right](1 - \PrTaken) \\
    & \equiv & \CorrValue{\PrTaken}{\PrVecP},
\end{eqnarray}
%
where we define this result to be $\CorrValue{\PrTaken}{\PrVecP}$, given \PrTaken and \PrVecP.
\end{proof}

%An additional useful fact is $\CorrValue{\PrTaken}{\PrVecP} = 1 - \CorrValue{1-\PrTaken}{\PrVecP}$.

For example, if all predictor states are initially equally likely, then $\PrWT=\PrST=\sfrac{1}{4}$ and $\SingleBranchMispred = 1 - \CorrValue{b}{[\sfrac{1}{4},\ldots,\sfrac{1}{4}]} = \sfrac{1}{2}$, which is independent of \PrTaken.
If instead the predictor always begins in either of the strongly or weakly taken states, then it must predict taken ($\PrWT+\PrST=1$) and $\SingleBranchMispred = 1 - \PrTaken$, as one would expect.

\subsection{Model for simple finite loops}
\label{sec:2-bit:model:for}

Consider the \emph{simple sequential while-loop} of \refalg{alg:loop}, which executes exactly $n$ iterations.%
  \footnote{That is, we assume (a) the iteration variable $i$ increases monotonically by 1 at each iteration; (b) the loop bound $n$ is constant as the loop executes; and (c) there are no early exits.}
The conditional branch in this case evaluates the condition, $i < n$, and takes the branch only when this condition is false.
There will be exactly $n+1$ evaluations of this branch.%
  \footnote{There is an additional branch at the bottom of the loop. However, this branch is unconditional, since it \emph{must} jump back to the top of the loop.}

%------------------------------------------------------------
\begin{algorithm}[t]
  Let $n \geq 0$\;
  $i \leftarrow 0$\;
  \While(\ \tcp*[h]{Initial state: \PrVecPi}){$i < n$}{
    \tcp*[h]{\ldots\ $i$, $n$ unmodified; no early exits \ldots}
    $i \leftarrow i + 1$\;
  }
  \caption{A simple sequential while-loop, which executes exactly $n$ iterations of its body}
  \label{alg:loop}
\end{algorithm}
%------------------------------------------------------------

How many of these $n+1$ conditional branches are mispredicted?
The following lemma tells us.

\begin{lemma}
  Consider a simple sequential while-loop of \refalg{alg:loop}, which executes $n$ iterations.
  If a 2-bit conditional branch predictor begins in an initial state $\PrVecP = [\PrSNT, \PrWNT, \PrWT, \PrST]$, then the expected number of mispredictions, considering only the loop termination checks, is \SimpleLoopMispred{n}{\PrVecP}, where
  \begin{eqnarray*}
    \SimpleLoopMispred{n}{\PrVecP} & = & \left\{\begin{array}{rl}
        1 - (\PrWT + \PrST)  &  n = 0 \\
                  1 + \PrWT  &  n = 1 \\
         1 + \PrWT + 2\PrST  &  n \geq 2
      \end{array}\right.
    .
  \end{eqnarray*}
\end{lemma}

\begin{proof}
Let $\CORR_i$ be the event that the conditional branch at $i$ is predicted correctly, where $0 \leq i \leq n$.
These events are independent since the outcome of the branch should depend only on $i$.
Thus, if we can compute their probabilities, we can compute their expected values, $\Expect{\CORR_i}$;
then the expected number of mispredictions will be $n+1-\sum_i{\Expect{\CORR_i}}$.
Defining $\CORR_i=1$ as ``correct'' and $\CORR_i=0$ as ``incorrect,'' then $\Expect{\CORR_i}=\Prob{\CORR_i}$.

This probability may be computed as follows.
Let \PrVecPi be the state probabilities row-vector just before the conditional branch of iteration $i$ executes, where $\PrVecPfirst$ is the initial state probabilities row-vector, before evaluating \emph{any} branches.
%let its value be $\PrVecPfirst \equiv [\PrSNT, \PrWNT, \PrWT, \PrST]$.
For all $i < n$, the branch is not taken so that $\Prob{\CORR_i} = \CorrValue{0}{\PrVecPi}$.
On the last branch, $i \geq n$ and we must exit the loop;
therefore, the last branch is taken and $\Prob{\CORR_n} = \CorrValue{1}{\PrVecPlast}$.
Similarly, the state probabilities are $\PrVecPi = \PrVecPim \PrTransMatNT = \PrVecPfirst \PrTransMatNT^i$ for all $0 < i < n$;
and for the last branch, $\PrVecPlast=\PrVecPlastTaken\PrTransMatT$.
Therefore, knowing only \PrVecPfirst and $n$, we may compute all \Prob{\CORR_i}.

These cases may be further simplified, since
%
\begin{eqnarray}
  \PrVecP \PrTransMatNT
    & = & [\PrSNT + \PrWNT, \PrWT, \PrST, 0] \\
\mbox{and\ }
  \PrVecP \PrTransMatT
    & = & [0, \PrSNT, \PrWNT, \PrWT + \PrST].
\end{eqnarray}
%
That is, the effect of \PrTransMatNT is to ``shift'' probability toward the strongly not taken state, while \PrTransMatT shifts the probability toward the strongly taken state.
This fact implies, for instance, that $\PrVecPfirst \PrTransMatNT^k = [1, 0, 0, 0]$ for all $k \geq 3$.
That is, after at most 3 iterations, the predictor must enter the strongly not taken state, just as \reffig{fig:branch-pred-fsa} suggests.

Taken together, the preceding facts (after some algebra) imply the lemma.
\end{proof}

As an example, suppose the initial states are equally likely just prior to the loop.
Then, $\SimpleLoopMispred{n}{[\sfrac{1}{4},\ldots,\sfrac{1}{4}]}$ is $\sfrac{1}{2}$ for $n=0$, $1\sfrac{1}{4}$ for $n=1$, and $1\sfrac{3}{4}$ for $n \geq 2$.

% eof

